Differentially Private In-context Learning via Sampling Few-shot Mixed with Zero-shot Outputs

In-context learning (ICL) has shown promising improvement in downstream task adaptation of LLMs by augmenting prompts with relevant input-output examples (demonstrations). However, the ICL demonstrations can contain privacy-sensitive information, which can be leaked and/or regurgitated by the LLM output. Differential Privacy (DP), a widely adopted privacy safeguard, has emerged to mitigate this privacy leakage, with recent work demonstrating strong privacy-utility tradeoffs in classification tasks for ICL. However, generation tasks for ICL are challenging due to the high-dimensional output space of open-ended generation. To this end, we propose $\texttt{dps-mozo}$, Differentially Private Sampling by Mixing One-shot with Zero-shot Outputs, a decoding framework that generates DP text by sampling from the product of multiple one-shot outputs mixed with a zero-shot output. This mixing effectively reduces the amount of information that can be leaked by each demonstration. By utilizing the inherent randomness in sampling from the mixed distributions, we can achieve DP without adding noise, thereby improving the privacy-utility tradeoff. Our experimental evaluations show $\texttt{dps-mozo}$ can achieve a strong privacy guarantee, $\epsilon=2$, with minimal utility degradation compared to non-private few-shot learning, $\textbf{0.3}$% ROUGE-L F1 score decrease on the SAMSum dataset with Gemma 2 2B.

==> algorithms/dps_mozo_alg2.tex <==
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
    \caption{\dpsmozo{}: Differentially Private Sampling}
    \label{alg:dpsmozo}
    \KwIn{LLM $\theta$, a set of input-output examples $D$, an input query $\mathbf{x}$, current output query $\mathbf{y}_t$, number of top public indices $k$, Renyi order $\alpha$, max generation size $T_{\max}$, number of shots $n_{\text{shots}}$} 
    \KwOut{output query $\mathbf{y}$}
    $\mathbf{y} \gets []$\;
    
    \For{$t=1, ..., T_{\max}$}
        {
        $S_t \gets$ Sample $n_{\text{shots}}$ without replacement from D\;
        
        \textcolor{blue}{// Public top-k indices selected from zero-shot output}
        
        $K \gets$ top-k indices from $\text{logit}_{\theta}(\mathbf{x}, \mathbf{y}_{<t})$ \alglinelabel{line:top-k} \;
        
        \textcolor{blue}{// Truncate zero-shot output with public indices}\;
        
        $\text{logit}_{\theta}(y_t | \mathbf{x}, \mathbf{y}_{<t}) \gets -\infty$ $\forall y_t \in K$ \alglinelabel{line:zero_shot} \;
        
        \For{$(\mathbf{x}_i, \mathbf{y}_i)\in S_t$}
        {
            \textcolor{blue}{// Truncate one-shot output with public indices} \;
            
            $\text{logit}_{\theta}(y_t |\mathbf{x}_i, \mathbf{y}_{i}, \mathbf{x}, \mathbf{y}_{<t})= -\infty$ $\forall y_t \in K$ \alglinelabel{line:post_trunc} \;
            
            \textcolor{blue}{// Bound divergence of mixed output distribution} \;
            
            $\overline{p}_{\theta, \lambda_i}(\mathbf{x}_i, \mathbf{y}_{i}, \mathbf{x}, \mathbf{y}_{<t}) \!\gets\! \sigma(\lambda_i \text{logit}_{\theta}(\mathbf{x}_i, \mathbf{y}_{i}, \mathbf{x}, \mathbf{y}_{<t}) \newline + (1-\lambda_i)\text{logit}_{\theta}(\mathbf{x}, \mathbf{y}_{<t}))$ \alglinelabel{line:mix} \;
            
            $\textstyle \lambda_i \gets \argmax_{\lambda\geq0} D_{\alpha}^{\leftrightarrow}(\overline{p}_{\theta, \lambda_i}(\mathbf{x}_i, \mathbf{y}_{i}, \mathbf{x}, \mathbf{y}_{<t}) || \newline p_{\theta}(\mathbf{x},$ $\mathbf{y}_{<t})) \leq \beta\alpha$ \alglinelabel{line:set_lambd} \;
        }
        
        $y_{t} \sim \prod_{i=1}^{n} \overline{p}_{\theta, \lambda_i}(y_t |\mathbf{x}_{i}, \mathbf{y}_i, \mathbf{x}, \mathbf{y}_{<t})$ \alglinelabel{line:ensemble} \;
        
        $\mathbf{y} \gets \mathbf{y} + [y_t]$\;
        
        \uIf{$y_t == \texttt{<eos>}$}{
            \KwRet{$\mathbf{y}$}
        }
    }
    \KwRet{$\mathbf{y}$}
\end{algorithm}
\end{minipage}
